Full-Rank No More: Low-Rank Weight Training for Modern Speech Recognition Models

This paper investigates the under-explored area of low-rank weight training for large-scale Conformer-based speech recognition models from scratch. Our study demonstrates the viability of this training paradigm for such models, yielding several notable findings. Firstly, we discover that applying a low-rank structure exclusively to the attention modules can unexpectedly enhance performance, even with a significant rank reduction of 12%. In contrast, feed-forward layers present greater challenges, as they begin to exhibit performance degradation with a moderate 50% rank reduction. Furthermore, we find that both initialization and layer-wise rank assignment play critical roles in successful low-rank training. Specifically, employing SVD initialization and linear layer-wise rank mapping significantly boosts the efficacy of low-rank weight training. Building on these insights, we introduce the Low-Rank Speech Model from Scratch (LR-SMS), an approach that achieves performance parity with full-rank training while delivering substantial reductions in parameters count (by at least 2x), and training time speedups (by 1.3x for ASR and 1.15x for AVSR).

==> tables/initialization_uniform.tex <==
\begin{table}[]
\centering
\captionsetup{font=scriptsize}
\caption{WER [\%] ($\downarrow$) of low-rank ASR models trained from scratch on LRS3. The models were initialized with different methods and uniform scaling factors were applied to the FFN.}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\textbf{$\alpha$} & \textbf{\# Params} & \textbf{Initialization} & \textbf{Test set} & \textbf{WER} \\ \midrule
0.5            & 189 M              & Kaiming                 & LRS3              & 2.58         \\
0.5            & 189 M              & SVD                     & LRS3              & 2.40         \\
\midrule
0.25           & 145 M              & Kaiming                 & LRS3              & 2.49         \\
0.25           & 145 M              & SVD                     & LRS3              & 2.41         \\
\midrule
0.12           & 122 M              & Kaiming                 & LRS3              & 2.37         \\
0.12           & 122 M              & SVD                     & LRS3              & 2.34        \\ \bottomrule
\end{tabular}
}
\label{tab:initialization}
\end{table}
